Artificial Intelligence for Smart Transportation

There are more than 7,000 public transit agencies in the U.S. (and many more private agencies), and together, they are responsible for serving 60 billion passenger miles each year. A well-functioning transit system fosters the growth and expansion of businesses, distributes social and economic benefits, and links the capabilities of community members, thereby enhancing what they can accomplish as a society. Since affordable public transit services are the backbones of many communities, this work investigates ways in which Artificial Intelligence (AI) can improve efficiency and increase utilization from the perspective of transit agencies. This book chapter discusses the primary requirements, objectives, and challenges related to the design of AI-driven smart transportation systems. We focus on three major topics. First, we discuss data sources and data. Second, we provide an overview of how AI can aid decision-making with a focus on transportation. Lastly, we discuss computational problems in the transportation domain and AI approaches to these problems.

==> Chapters_r2/background.tex <==
\section{Background}

TODO

==> Chapters_r2/context.tex <==
\section{Smart Cities Context}

Effective solutions are of critical importance in that poorly designed mobility applications can make for unhappy users, increase costs or in the case of safety critical applications can affect the livelihood of residents that depend on the system.
In this way, AI-driven transportation systems require high-quality datasets to train models and real-time ingestion and processing methods for inference.
\textcolor{red}{MW: provide a high level block diagram of a real-time transportation system}

%\subsection{Data Sources and Data Management}

\subsection{Static Data Sources}

Data sources can be classified as static or real-time data.
Static data are datasets related to the road networks, GIS layout and schedules for the operating regions while real-time data consists of data streaming from sensors and collected during real-time operations.
In this sense, the static data is not fully "static".
For instance, roadway information can get updates over time and fixed-line schedules can change.
However, the static data in this work is not required to be updated daily in the way that real-time data does.

\subsubsection{Roadway Infrastructure and Routing Graphs}

Transportation models require a way to represent the roadway network.
A commonly used roadway network data source is OpenStreetMap (OSM).
OSM is community-driven and open-source with updates provided by the OSM community with a wide geographic footprint \cite{haklay2008openstreetmap}.
Data can be directly downloaded from various mirrors \cite{geofabrik} and is used as the mapping data for a variety of commercial-grade applications.
OSM in its raw form consists of \textit{nodes} which are points with a geographic position (latitude, longitude), \textit{ways} which are ordered lists of nodes representing linear features such as streets and \textit{relations} which define relationships between nodes and ways.
Together, these features represent a graph which can be used for mapping or routing.
There are numerous open-source projects that provide routing services such as shortest path calculation and travel time estimation using OSM data including the Open Source Routing Machine (OSRM), OpenTripPlanner and Valhalla \cite{osrm, valhalla}.

\subsubsection{Transit Schedules}\label{subsubsection: transit schedules}

The most widely used schema for representing fixed-line routes and schedules is the General Transit Feed Specification (GTFS) \cite{staticgtfs}.
GTFS includes a standard format for public transportation schedules and associated geographic information.
This includes standard representations for routes, trips, stops and scheduled arrival times at each stop for buses and subway networks.
It also includes geospatial shape objects representing routes so that fixed-line transit can be mapped to the operating region.
Public transit agencies maintain and publish their own schedules in GTFS format for public consumption.
In this way, developers and researchers can write code that consumes GTFS data in an interoperable way that can work across transit agencies and regions, provided the transit agency maintains a GTFS-compliant data source.

\subsubsection{On-Demand Driver Runs}

Some forms of on-demand transportation, particularly those managed directly by public transit agencies, may include scheduling information for vehicles and drivers.
For instance, in the case of micro-transit and para-transit, a transit agency when maintain a list of available drivers for a day and the start and end times of their runs.
They may also maintain the list of available vehicles including the capacity of each vehicle and which driver run corresponds to each available vehicle.
This contrasts with many commercial ride-share settings such as Uber or Lyft where there are not fixed schedules for drivers or fixed vehicles each driver will use.

\subsection{Environment Sensing - Real-time Data Sources}

Advances in sensing technologies have led to an explosion of real-time streaming data in urban environments.
These sensors allow us to monitor transportation systems in real-time and act as a bridge between the physical and cyber domains.
They allow us to quantify and monitor the system through data.
Real-time data then serves two purposes.
First, we can collect sensor data over a time range to generate offline datasets.
These offline datasets are joined with the static data and used to train AI models.
Second, the learned models then ingest the sensor data at inference time to make predictions and aid the decision-making process.

The data itself comes in a variety of formats and is typically defined as high-velocity and high-volume.
Therefore, the problem of ingesting, processing, storing and interpreting real-time sensor data in the transportation domain inherits the traditional problems associated with Internet of Things (IoT) analytics \cite{mohammadi2018deep}.
In this section we outline commonly used real-time data sources in the transportation domain.

\subsubsection{Vehicle Telematics}\label{subsubsection: vehicle telematrics}

TODO

\subsubsection{GTFS Realtime}

As discussed in \ref{subsubsection: transit schedules}, GTFS is an open data format used by many transit agencies to represent public transportation schedules and associated geographic information.
GTFS Realtime is an extension to the static GTFS schedules that provides up-to-date information about current arrival times, vehicle locations, occupancy and service alerts to help users better plan their trips \cite{realtimegtfs}.
The structured nature of GTFS Realtime makes it easy to monitor fixed-line public transit performance in the context of the transit schedules and routes.
GTFS Realtime has been incorporated in a variety of commercial-grade applications including Google Maps.
GTFS Realtime typically is provided by transit agencies themselves.
Compared to raw GPS as discussed in section \ref{subsubsection: vehicle telematrics}, GTFS Realtime is a structured format that is interoperable between agencies and telematics kit providers.

\subsubsection{Weather}

TODO

\subsubsection{Traffic}

TODO


%There are numerous challenges in storing and processing data for building AI models in the transportation domain. 
%First, these sources present data in domain-specific formats and at irregular intervals that can vary by provider and source, making it challenging to join data streams to be used by downstream applications \cite{wang2000spatiotemporal}. 
%Second, the spatiotemporal nature of these data sources presents challenges in efficient storage, synthesis and data retrieval \cite{aydin2016modeling}, \cite{wang2019integrated}. 
%A third challenge is efficiently representing and presenting the data in ways that can be used by domain experts \cite{thudt2013visits}. 
%In addition, there are the typical challenges of working with high-velocity, high-volume streaming data.



==> Chapters_r2/intro.tex <==
\section{Introduction}

There are more than 7,000 public transit agencies in  the U.S. (and many more private agencies), and together, they are responsible for serving 60 billion passenger miles each year.
Additionally, new on-demand modalities including ride-share, bike-share and e-scooters have been introduced in recent years and transformed the transportation landscape in urban environments.
A well-functioning transit system fosters the growth and expansion of businesses, distributes social and economic benefits, and links the capabilities of community members, thereby enhancing what they can accomplish as a society~\cite{beyazit2011evaluating,harvey2010social,federal2003status}. 
However, the explosion in transportation options and complicated relationship between public and private offerings present myriad new challenges in the design and operation of these systems.
There are also complex, and often competing, operational objectives that complicate the implementation of efficient services.
Affordable public transit services are the backbones of many communities.
Solving these problems and understanding state-of-the-art methods for AI-driven smart transportation has the potential to strengthen urban communities, address the climate challenge and foster equitable growth.


Fundamentally, the design of well-functioning transit systems require solving complex combinatorial optimization problems related to planning and real-time operations.
These problems span many well studied fields including classical line planning, offline and online vehicle routing problems (VRPs).
While there are many ways to evaluate the performance of smart transportation systems, we largely focus on evaluating these systems in the context of optimizing \textit{utilization} (i.e. ridership) and \textit{efficiency} (i.e. reducing operational costs).
Increasing utilization requires learning mobility patterns over large-geographies and adapting systems to better meet demand.
It also requires flexible mobility options such as on-demand and multi-modal transportation to adapt to demand in real-time and thus better serve potential passengers.
Additionally, more efficient systems reduces the impact on the environment by reducing emissions and can free resources by reducing costs.
Lastly, \textit{coverage} is an important consideration that often competes with utilization and efficiency.
Therefore it is important to discuss optimization in the context of \textit{ridership} versus \textit{coverage}, the latter of which is an important consideration in the design of equitable and fair transportation.
While the ridership versus coverage problem is open-ended there are ways in which these dimensions can be modelled such that transit agencies can better optimize over the objectives that matter most to them.

Efficient transportation systems require making decisions in real-time over large geographies and computationally intractable state-action spaces.
Due to the intractability of these problems, traditional analytical methods fall short.
Therefore, transit agencies have turned to computational approaches that enable large-scale data-driven optimization.
AI-driven transportation can address this problem by learning complex abstractions of vast volumes of data to make decisions in a computationally efficient manner at scale and in real-time.
However, it requires solving complex challenges in model representation, decision-making uncertainty as well as data ingestion and processing.

%Designing efficient transportation systems involves solving intractably large problems in which traditional analytical methods fall short.
%Therefore, transit agencies have turned to computational approaches that enable large-scale data-driven optimization.

%In this way, AI algorithms can leverage complex abstractions of vast volumes of data to make decisions or model the environment in a computationally efficient manner that allows transit operators to solve problems at city-scale.
%However, there are numerous challenges associated with designing data-driven, or AI-driven transportation systems.
%First, transportation data is high-volume and high-velocity so there must be carefully designed data processing and ingestion methods for handling various structured and unstructured data.
%Second, smart transportation systems require making decisions in real-time over large geographies and computationally intractable state-action spaces.
%This requires computationally efficient environmental models and decision-making algorithms.


%Efficient transportation systems require making decisions in real-time over large geographies and computationally intractable state-action spaces.

Smart transportation is a broad field, therefore we primarily focus on two high-impact modalities; fixed-line and on-demand transportation systems.
Fixed-line transportation consists of a fixed schedule of vehicles (bus or rail) which will traverse pre-defined routes over the course of a day.
On-demand transportation is a flexible form of transportation in which users request rides in real-time or ahead-of-time and transportation is provided from point A to B through ride-share, e-scooters or bike-share.
Additionally, recently transit agencies have investigated the potential of multi-modal transportation which provides a more flexible and adaptive transportation model that combines fixed-line and on-demand transportation.

%This chapter outlines key challenges in these domains as well as the potential of multi-modal transportation for next generation transit which provides a more flexible and adaptive transportation model that combines fixed-line and on-demand transportation.

This chapter discusses the primary requirements, objectives and challenges related to the design of AI-driven smart transportation systems.
The major content involves the following:
\begin{enumerate}
    \item Data sources and data management for AI-driven transportation.
    \item Computational problems in the transportation domain and AI approaches.
\end{enumerate}



%A key component of all problems in this space is the balance between \textit{ridership} and \textit{coverage}. 
%Affordable public transit services are the backbones of many communities, providing diverse groups of people with access to employment, education, and other services.
%Affordable transit services are especially important in low-income neighborhoods where residents might not be able to afford personal vehicles.
%However, transit services that provide wide and equitable coverage tend to suffer from low utilization---compared to concentrating service into a few high-density areas---which leads to higher fuel usage per passenger per mile.
%This in turn results in higher operating costs, which  threatens affordability---a problem that has recently been exacerbated by the COVID-19 pandemic.

==> energy_assignment/simulated_annealing.tex <==
\subsection{Simulated Annealing}
\label{sec:annealing}

Finally, we introduce a simulated annealing algorithm, which improves upon the output of the greedy algorithm  using iterative random search.
Starting from a greedy solution, the search takes significantly less time than starting from random solution. % (compared to starting with a random solution).
The key element of this algorithm is choosing a random ``neighboring'' solution in each iteration.



\begin{algorithm}[ht]
 \caption{$\textbf{RandomNeighbor}(\mathcal{A}, p_{swap})$}
 \label{algo:mutation}
     $\textit{NumberOfSwaps} \leftarrow \textbf{max}\{1, |\mathcal{A}| \cdot p_{swap}\}$
     
    \For {$1, \ldots, \textnormal{\textit{NumberOfSwaps}}$}
    {
     $v_1, v_2 \leftarrow \textbf{UniformRandom}(\mathcal{V})$
     
     $\mathcal{T}_1 \leftarrow \{{t} \in \mathcal{T} ~|~ \langle v_1,{t} \rangle \in \mathcal{A}\}$
     
    $\mathcal{T}_2 \leftarrow \{{t} \in \mathcal{T} ~|~ \langle v_2,{t} \rangle \in \mathcal{A}\}$
    
    $\textnormal{\textit{SplitTime}} \gets \textbf{UniformRandom}([s_1^{start}, s_\infty^{end}])$
     
    $\mathcal{T}_{noswap}, \mathcal{T}_{swap} = \textbf{SplitByStartTime}(\{\mathcal{T}_1, \mathcal{T}_2\}, \textnormal{\textit{SplitTime}})$
    
    \For{$t \in \mathcal{T}_{swap}$}
    { 
        \uIf{$t \in \mathcal{T}_1$}
        {
           $\mathcal{A} \leftarrow \mathcal{A} \setminus \{\langle v_1, t \rangle\} \cup  \{\langle v_2, {t} \rangle\}$
        }
        \Else %If{$t \in \mathcal{T}_2$}
        {
          $\mathcal{A} \leftarrow \mathcal{A} \setminus \{\langle v_2, t \rangle\} \cup \{ \langle v_1, {t} \rangle\}$
        }
        }

    }
    
 \KwResult{$\mathcal{A}$}
\end{algorithm}



\paragraph{Random Neighbor}
Simulated annealing uses \cref{algo:mutation} to generate a random  neighbor for a candidate solution $\mathcal{A}$. The algorithm first chooses two vehicles $v_1,v_2$ at random from $\mathcal{V}$. Next, the algorithm enumerates all the trips $\calT_1$ and $\calT_2$ that are assigned to these vehicles in solution $\calA$,
chooses a random point in time $\textit{SplitTime}$ during the day, and splits all these trips into two sets $\mathcal{T}_{noswap}$ and $\mathcal{T}_{swap}$ based on the start times of the trip and $\textit{SplitTime}$.
Finally, the algorithms swaps all the trips in $\mathcal{T}_{swap}$ between $v_1$ and $v_2$ (i.e., trips that were assigned to $v_1$ are re-assigned to $v_2$ and vice versa).
The algorithm then repeats this process from the beginning until the desired number of swap operations $|\mathcal{A}| \cdot p_{swap}$ is reached. 
% The time complexity of this algorithm is $\mathcal{O}\left(|\calA|\cdot(|\calT|+|\calV|)\right)$.



\begin{algorithm}[!h]
 \caption{$\textbf{Simulated Annealing}(\mathcal{V}, \mathcal{T}, \mathcal{C},  \alpha, k_{max}, \newline p_{start}, p_{end}, p_{swap})$}
 \label{algo:sti_mul_anneal}

$\mathcal{A} \leftarrow \textbf{Greedy}(\mathcal{V}, \mathcal{T}, \mathcal{C}, \alpha)$

$\textnormal{\textit{Solutions}} \leftarrow \{ \mathcal{A} \}$

$\tau_{start} \leftarrow \frac{-1}{\ln{p_{start}}}$

$\tau_{end} \leftarrow \frac{-1}{\ln{p_{end}}}$

$\tau_{rate} \leftarrow \left(\frac{\tau_{end}}{\tau_{start}}\right)^{\frac{1}{k_{max} -1}} $

$\tau_{k} \leftarrow \tau_{start}$

$\delta_{avg} \leftarrow 0$

%$k \leftarrow 0$

 \For {$k = 1, 2, \ldots, k_{max}$}
 {  
    
    $\mathcal{A'} \leftarrow \textbf{RandomNeighbor}(\mathcal{A}, p_{swap})$


    $\delta_e \leftarrow \textbf{Cost}(\mathcal{A'}) - \textbf{Cost}(\mathcal{A})$
    
    \If{k = 1}
    {
        $\delta_{avg} \leftarrow \delta_e$
    }
    
    $\textit{AcceptProbability} \leftarrow \exp{\left(\frac{-\delta_e}{\delta_{avg} \cdot \tau_k}\right)}$
    

    \If{$\textnormal{\textbf{Cost}}(\calA') < \textnormal{\textbf{Cost}}(\calA)  ~\textnormal{\textbf{or}}~ \textit{AcceptProbability} > \textnormal{\textbf{UniformRandom}}([0,1])$}
    {
    
     $\mathcal{A} \leftarrow  \mathcal{A'}$
     
    $\delta_{avg} \leftarrow \delta_{avg} + \frac{\delta_e - \delta_{avg}}{|Solutions|} $
          
     $\textnormal{\textit{Solutions}} \leftarrow \textnormal{\textit{Solutions}} \cup \{\mathcal{A}\}$
    }
     
     $\tau_{k} \leftarrow \tau_{k} \cdot \tau_{rate}$   
 }
 
 $\calA^* \gets \argmin_{\calA' \in \textnormal{\textit{Solutions}}} \textbf{Cost}(\calA')$ 
 \KwResult{$\calA^*$} 
\end{algorithm}



\cref{algo:sti_mul_anneal} shows our simulated annealing approach.
First, the algorithm obtains an initial solution $\mathcal{A}$ using \cref{algo:greedy_approach}. Then, it follows an iterative process. In each iteration, the algorithm obtains a random neighboring solution $\mathcal{A}'$ of the current solution $\mathcal{A}$ using \textbf{RandomNeighbor}. If the energy cost \textbf{Cost} (see \cref{equ:obj_main}) of $\mathcal{A}'$ is lower than the energy cost of $\mathcal{A}$, then the algorithm always accepts $\mathcal{A}'$ as the new solution. Otherwise, the algorithm computes the probability $\textit{AcceptProbability}$ of accepting it based on a decreasing temperature value $\tau_k$ and the cost difference between $\calA'$ and $\calA$, and then accepts $\calA'$ at random.
The algorithm terminates after a fixed number of iterations $k_{max}$ and returns the best solution found up to that point.
% The time complexity of this algorithm is $\mathcal{O}\left(k_{max}\cdot |\calT|\cdot(|\calT|+|\calV|)\right)$.


==> impact.tex <==
\section{Social Impact}

description of the impact (or projected impact)


==> main_r2.tex <==
% \documentclass[acmsmall, nonacm]{acmart}
% \usepackage[utf8]{inputenc}

% \usepackage{xcolor}

% \usepackage{amsmath}
% \usepackage{mathtools}

% \usepackage[ruled,noend]{algorithm2e}
% \usepackage{algpseudocode}

% \newcommand{\calA}[0]{\ensuremath{\mathcal{A}}}
% \newcommand{\calC}[0]{\ensuremath{\mathcal{C}}}
% \newcommand{\calE}[0]{\ensuremath{\mathcal{E}}}
% \newcommand{\calL}[0]{\ensuremath{\mathcal{L}}}
% \newcommand{\calM}[0]{\ensuremath{\mathcal{M}}}
% \newcommand{\calN}[0]{\ensuremath{\mathcal{N}}}
% \newcommand{\calS}[0]{\ensuremath{\mathcal{S}}}
% \newcommand{\calT}[0]{\ensuremath{\mathcal{T}}}
% \newcommand{\calX}[0]{\ensuremath{\mathcal{X}}}
% \newcommand{\calV}[0]{\ensuremath{\mathcal{V}}}
% \newcommand{\calTN}[0]{\ensuremath{\mathcal{T'}}}
% \newcommand{\calEC}[0]{\ensuremath{\mathcal{EC}}}

% \newcommand{\argmax}[0]{\ensuremath{\operatorname{argmax}}}
% \newcommand{\argmin}[0]{\ensuremath{\operatorname{argmin}}}

% \usepackage[size=tiny]{todonotes}
% \newcommand{\sidenote}[1]{\todo[color=yellow!10, linecolor=yellow!50!black]{#1}}

% \newenvironment{copypasted}{\color{blue!50!black}}{\color{black}}

% \usepackage[capitalize]{cleveref}

% \title{AI for Smart Transportation}

% \author{Samitha Samaranayeke}
% \affiliation{\institution{Cornell University}
% \country{USA}
% }

% \author{Abhishek Dubey}
% \affiliation{\institution{Vanderbilt University}
% \country{USA}
% }

% \author{Aron Laszka}
% \affiliation{\institution{Pennsylvania State University}
% \country{USA}
% }

% %\institute{Cornell University \and Vanderbilt
% %University \and Pennsylvania State University}

% \begin{document}

% %\setcounter{tocdepth}{2}
% %\tableofcontents
% %\clearpage

% \maketitle

% \input{Chapters_r2/intro}

% \input{Chapters_r2/context}

% \input{Chapters_r2/background}


% \bibliographystyle{plain}
% \bibliography{main.bib}

% \end{document}
